Hazards in Deep Learning Testing: Prevalence, Impact and Recommendations

Much research on Machine Learning testing relies on empirical studies that evaluate and show their potential. However, in this context empirical results are sensitive to a number of parameters that can adversely impact the results of the experiments and potentially lead to wrong conclusions (Type I errors, i.e., incorrectly rejecting the Null Hypothesis). To this end, we survey the related literature and identify 10 commonly adopted empirical evaluation hazards that may significantly impact experimental results. We then perform a sensitivity analysis on 30 influential studies that were published in top-tier SE venues, against our hazard set and demonstrate their criticality. Our findings indicate that all 10 hazards we identify have the potential to invalidate experimental findings, such as those made by the related literature, and should be handled properly. Going a step further, we propose a point set of 10 good empirical practices that has the potential to mitigate the impact of the hazards. We believe our work forms the first step towards raising awareness of the common pitfalls and good practices within the software engineering community and hopefully contribute towards setting particular expectations for empirical research in the field of deep learning testing.

==> pages/7-related.tex <==
\section{Related work}
\label{sec:related}

% On Evaluating Adversarial Robustness: https://nicholas.carlini.com/papers/2019_howtoeval.pdf
% Dos and Don'ts of Machine Learning in Computer Security: https://arxiv.org/pdf/2010.09470.pdf?
% A survey of deep active learning
% Machine learning testing: Survey, landscapes and horizons
% Testing machine learning based systems: a systematic mapping

==> pages/discussion.tex <==
\subsection{Dataset collection and preparation}
\paragraph{Multiple datasets} - \textbf{Important}:

\textbf{Description.} Whether the paper base its claims on diverse datasets. The diversity includes the size of the datasets in terms of features and number of examples. 


\textbf{Recommendations.} When applicable, the evaluation should cover multiple domains and tasks. In particular, while the main evaluation could be restricted to simple datasets like CIFAR10, challenging datasets should be included in the evaluation of the main claims. Challenging datasets include ImageNet, COCO or Cityscapes for image detection and classification, and GLUE [] and NewsQA [] for NLP tasks. Simple datasets like MNIST (and its variants) should only be considered as toy examples. 

\textbf{Assessment.}
\begin{itemize}
\item Absent: The paper only evaluates small datasets in one domain (generally Computer Vision)

\item Fair: The paper evaluates small and large datasets in one domain

\item Adequate: The paper evaluates small and large datasets in multiple domains
\end{itemize}

\paragraph{Datasets split} - \textbf{Important}: 

\textbf{Description.} Whether the paper splits the train/test and sampled the seed inputs. When the objective of the paper is to generate buggy inputs, it is critical to ensure that the initial seeds used to generate the buggy inputs are not initially buggy. Indeed, generating new bugs for ML systems is straightforward starting from inputs with incorrect behaviours. Adding small perturbations around these inputs following the loss of the model leads to inputs that are also buggy.    

\textbf{Recommendations.} To assess the effectiveness of an approach in generating new buggy inputs, the first consideration is that the seeds of the approach should be benign inputs for the model. The seeds should be sampled from the correctly behaving inputs. In addition, if the generated inputs are used to improve the model (by retraining or repair), it is critical that the final evaluation of the model before deployment should use an independent set that was not used to seed the newly generated inputs. The preferred practice is to only use the training set to sample the seeds used to generate the additional test examples.

\textbf{Assessment.}
\begin{itemize}
     \item Absent: The sampled seeds to generate inputs are limited, or already problematic 

\item N/A: for papers targeting only detection of samples

\item Unknown: Unclear from paper and source code

\item Fair: Used benign seed inputs

\item Adequate: Used all the non-buggy test set as seed inputs; kept a subset of test input separate for independent evaluation
\end{itemize}


\paragraph{Class imbalance} - \textbf{Important} : 

\textbf{Description.} Whether the class imbalance of the dataset is correctly handled. Imabalanced datasets can lead to misleading results when the appropriate metrics are not evaluated.

\textbf{Recommendations.} Unbalanced datasets can be handled at 2 different levels. At the evaluation level, using the appropriate metrics according the severity of the unbalance. Metrics like the Area Under ROC curve (AUC) or the Matthews correlation coefficient (MCC) are recommended. The AUC takes into account cases where the classification threshold can significantly impact the performances of the model. Improving the AUC reflects both an improvement of the True Positive Rate (TPR) and the False Positive Rate (FPR) which better reflect the performances of an unbalanced dataset.  
MCC is also a more reliable statistical rate which produces a high score only if the prediction obtained good results in all of the four confusion matrix categories. MCC is recommended for extremely imbalanced datasets like cyber-security or healthcare tasks.

Class imbalance can also be mitigated during training and evaluation with an optimal weighting or thresholding of the contribution of each classes to the loss. Class imbalance can also be mitigated using data sampling or augmentation to reduce or cancel the imbalance.

\textbf{Assessment.}
\begin{itemize}
     \item Absent: The datasets studied exhibits clear class imbalance that was not considered

     \item N/A: The datasets studied do not exhibit any class imbalance

     \item Unknown: The datasets studied exhibit clear class imbalance but its mitigation is unclear from paper and source code

     \item Fair: The class imbalance of the datasets is acknowledged with imbalanced datasets metrics

     \item Adequate: The class imbalance of the datasets is mitigated (with sampling, loss weighing, class-specific thresholds….)
\end{itemize}


\subsection{Randomness}
\paragraph{Repetitions} - \textbf{Important}: 

\textbf{Description.} Whether the paper provides multiple repetitions for critical experiments

\textbf{Recommendations.} Training and evaluating deep learning models inherently measures and optimizes metrics across thousands of inputs. While the training process is also stochastic, the use of multiple batches and epochs amounts to repeating the training process. In addition, SoTA robustness attacks and defense include inherently repetition mechanisms. Therefore repeating critical experiments is only needed when the evaluation set is small, when the training/fine-tuning is done across few epochs, or when the proposed methods introduce randomness that would not be counter-balanced by the the multiple seeds and inputs evaluated.  

\textbf{Assessment.}
\begin{itemize}
    \item Absent: The paper does not repeat any experiment, or repeats with the same seed.

    \item Fair: The paper repeats the most critical experimental parts or demonstrates that repetition has little impact on the core of the experiments

    \item Adequate: The paper evaluates all experiments with multiple repetitions
\end{itemize}


\paragraph{Statistical significance} - \textbf{Important}: Whether the paper evaluation statistical significance when repeating experiments, comparing methods or analyzing correlations

\textbf{Recommendations.} Similarly to the repetition criteria, statistical significance is required when the randomness introduced by the paper's approaches is not balanced by the evaluation protocol. In particular when the improvements claimed by the methods are marginal, or when the conclusions of the paper differ from one setting (dataset, model, ...) to another. 

\textbf{Assessment.}
\begin{itemize}
    \item Absent: The paper does not provide any statistical significance study.

    \item Fair: The paper provides for the most critical experiments / claims a statistical significance study

    \item Adequate: The paper evaluates a statistical significance of all experiments 
\end{itemize}



\subsection{Scope and threat model}

\paragraph{Clear definition} - \textbf{Important}: 

\textbf{Description.} If the paper clearly states what is the use case and what is the scenario evaluated (whitebox, graybox, blackbox). The baselines and the SoTA need to match the scope and threat model.

\textbf{Recommendations.} xxxx

\textbf{Assessment.}
\begin{itemize}
    \item Absent: No scope and threat model stated

    \item Fair: The scope or the threat models are stated

    \item Adequate: The scope or the threat models are stated and the impact of different threats models on the results are evaluated or discussed.
\end{itemize}

        \paragraph{Adaptive evaluation} - \textbf{Important}: 

\textbf{Description.} If the paper proposes a new technique to generate bugs, it needs to assume a model aware of this technique (either trained with examples from this technique, or that obfuscate / hinder the techniques used); if the paper proposes a technique to improve performances, adaptive attacks that consider the improvement scheme should be evaluated. 

\textbf{Recommendations.} xxxx

\textbf{Assessment.}
\begin{itemize}
    \item Absent: No adaptive generation or robustification technique considered

    \item Fair: The impact of adaptive generation or robustification is discussed

    \item Adequate: The impact of adaptive generation or robustification is evaluated
\end{itemize}

\paragraph{Computation cost} - \textbf{Important}: 

\textbf{Description.} Whether the paper evaluates the impact of its proposed methods in terms of computation cost, especially to generate the additional examples.

\textbf{Recommendations.} The evaluation should either demonstrate that under lower computation the proposed approach works well, or under high computation it outperforms SoTA; but not comparing their approach with reasonable budget techniques (eg. FGSM[] or PGD[]).

\textbf{Assessment.}
\begin{itemize}
    \item Absent: No assessment of the impact of budget on the results

    \item Fair: Ablation / comparative experiments on the impact of budget on the results

    \item Adequate: Comparison with SoTA under the same budgets
\end{itemize}


\paragraph{Pareto evaluation} - \textbf{Important}: 

\textbf{Description.} Retraining on the generated examples should be evaluated on the original distribution test (correctness) as well as the rest of generated examples (robustness / generalization). It is known there is a tradeoff between both[], and models that may exhibit good improvements in the latter can be totally unusable on the original test distribution.

\textbf{Recommendations.} Whenever the model is altered using the generated test cases, both the performance of the model on new generated cases, and on a independent test should be evaluated and reported separately. 

\textbf{Assessment.}
\begin{itemize}
    \item Absent: No evaluation on original test distribution

    \item N/A: The paper does not retrain its models

    \item Fair: Evaluation on both original distribution and artificial distribution

    \item Adequate: evaluation on original distribution and multiple distributions (proposed approach, adversarials, OOD)
\end{itemize}



\paragraph{Hyper-parameters tuning}: 

\textbf{Description.} For the papers that compare to fair or adequate baselines, whether the hyper-parameters of these baselines and the paper's approach have been tuned to the paper’s study. 

\textbf{Recommendations.} xxxx

\textbf{Assessment.}
\begin{itemize}
    \item Absent: No or incorrect baselines or absent HP consideration of baselines

    \item Fair: HP of baselines considered / discussed

    \item Adequate: multiple HP evaluated or HP tuned in the baselines for best results
\end{itemize}

\paragraph{SoTA evaluation techniques}: 

\textbf{Description.} The SoTA in adversarial input generation, detection and robustification has stabilized in the recent years with established attacks, detectors, defenses and benchmarks.   

\textbf{Recommendations.} If the paper used the relevant SoTA for comparison; Strong attacks for bug generation papers (AutoAttack), strong detectors (LID, RCE, …) for input detection, TRADES for robustification without correctness degradation.

\textbf{Assessment.}
\begin{itemize}
    \item Absent: No or irrelevant baselines 

    \item Fair: Outdated baselines evaluated

    \item Adequate: SoTA baselines evaluated
\end{itemize}


\section{Extra considerations and recommendations}



